Inventories, Demand Shocks Propagation and Amplification in Supply Chains

I study the role of industries' position in supply chains in shaping the transmission of final demand shocks. First, I use a novel shift-share design leveraging destination-specific final demand shocks and a new measure of destination exposure accounting for direct and indirect linkages. I find that demand shocks amplify significantly as they propagate upstream, with upstream industries experiencing output elasticities up to three times larger than final good producers, consistent with the bullwhip effect. To rationalize these empirical results, I develop a tractable production network model with inventories and study how the properties of the network and the cyclicality of inventories interact to determine whether final demand shocks amplify or dissipate upstream. I test the mechanism by directly estimating the model-implied relationship between output growth and demand shocks, mediated by network position and inventories. I find that the presence of inventories increases output elasticities by 18% on average, highlighting the macroeconomic significance of this channel. Finally, I use the model to quantitatively study the effects of long-run trends of lengthening supply chains and rising inventories on the volatility of the economy.

==> input/quantmodel.tex <==

\section{Endogenous Inventory Policy}\label{quantmodel_sec}

The economy is populated by a representative agent with stochastic demand.\footnote{This is equivalent to stochastic income and linear preferences.} The demand process follows some AR(1) with a drift $\bar D$ and persistence $\rho$. The error term is normally distributed with zero mean and some standard deviation $\sigma$. Denote the level of final demand as $y(\epsilon)$ where $\epsilon$ is the realization of the error term.

Firms produce the consumption good using inputs from outside the model. Producers face a time-to-sell constraint such that their sales $y\leq s+\chi q$, where $s$ denote the beginning of the period inventories, $q$ denotes output and $\chi\in(0,1)$ governs the intensity of the time-to-sell friction. Crucially, firms make production decisions before the uncertainty about current demand is unraveled. 
Sales are then given by the minimum between the quantity demanded by consumers and the available amount, such that $y=\min\{ s+\chi q,y(\epsilon)\}$. Firms also face a stock-out penalty $b$, which occurs whenever the firm is unable to satisfy consumer demand fully. This assumption stands in for the punishment that consumers may inflict on a firm if they have to incur additional search costs to find new suppliers of the good.
Given this setting the law of motion of inventories is given by
%
\begin{align*}
    s^{\prime}=s+q-y=s+q-\min\{ s+\chi q,y(\epsilon)\}.
\end{align*}
Namely, next-period inventories are given by current inventories plus current output minus sales, which are the minimum between consumer demand and current inventories plus the fraction of current output that can be sold today. 
The firms current payoffs are given by
%
\begin{align*}
    \pi(s,\epsilon_{-1})=-cq+p\mathbb{E}[\min\{s+\chi q,y(\epsilon)\}],
\end{align*}

Where $c$ is the price of inputs and $p$ that of output. 
Note that the choice of production is made before uncertainty realises, hence the lagged shock as a state variable and the expectation operator on the current state of demand. 

Including the stock-out penalty and writing the problem recursively:
%
\begin{align*}
    V(s,\epsilon_{-1})=\max_{q} -cq+p\mathbb{E}(y) -b Pr(y(\epsilon)>s+\chi q )+\beta \mathbb{E}V(s^\prime,\epsilon).
\end{align*}

\paragraph{Results}

I solve for the optimal policy and simulate the economy 2000 times for 960 periods. The first 240 periods are dropped to evaluate the behavior in steady state.
Recall that in the NBER CES sample I observe end-of-year inventories and yearly sales. To keep the model moments closer to the data counterparts, I report them in two versions: one in which I take every period to be a month and use all available periods; and one in which I pretend that I observe only yearly figures, hence the flows are aggregated over 12 periods while the inventory stock is observed only every 12th period. Therefore, the reported statistics are for 720 months and 60 years, respectively.

The model parameters are reported in Table \ref{parameter}. The key results concern the inventory behavior and volatility of output and sales, relative to that of the underlying stochastic process. These statistics are reported in Tables \ref{quantresults} and \ref{quantresults2}. As in the main body, define $\alpha_i=I^i/\mathbb{E}Y^i$, where $Y^i$ denotes sales. 

% \begin{table}[H]
%     \centering
%     \begin{tabular}{c|c}
%     \toprule 
%     Parameter & Value\\
%     \midrule
%         $p$ &3  \\
%         $\beta$ & .95\\
%         $c^1$& 0.8\\
%         $c^2$& 0.4 \\
%         $\bar{D}$& 1\\
%         $\rho$ & 0.9\\
%         $\sigma$& 0.1\\
%         \bottomrule
%     \end{tabular}
%     \caption{Parameters}
%     \label{parameter}
% \end{table}


\begin{table}[htp]
    \centering
    \begin{tabular}{c| ccccccccc}
    \toprule 
    Parameter & $p$ & $\beta$ &$c$& $\chi$ & $b$&$\bar{D}$&$\rho$ &  $\sigma$ \\
        \midrule
    Value      &3 & .95&         0.3&     $.5$&    10 &         1&        0.9&       0.1\\
        \bottomrule
    \end{tabular}
    \caption{Parameters}
    \label{parameter}
\end{table}

\begin{table}[htp]

\begin{minipage}[b]{0.32\hsize}\centering
    \centering
    \begin{tabular}{c|c c c c }
    \toprule 
     & Mean & Min & Max & Corr with $q(\epsilon)$\\
    \midrule
        Monthly \\
\midrule

        $\alpha$& 0.95   &0.93 &   0.97 &-0.08\\
        $I$& & && 0.47 \\
        \midrule
                Yearly \\
\midrule
                $\alpha$& 0.077   &0.076 &   0.079 &-0.037\\
        $I$& & && 0.27 \\
        \bottomrule
    \end{tabular}
    \caption{Levels}
    \label{quantresults}
\end{minipage}
% \end{table}
    \hspace{150pt}
% \begin{table}
\begin{minipage}[b]{0.32\hsize}\centering
    \centering
    \begin{tabular}{c|c  }
    \toprule 
     & $\sigma/ \sigma_{q(\epsilon)}$\\
    \midrule
    Monthly \\
    \midrule
        $Y$&1\\
        $Q$&2.19\\
            \midrule
    Yearly \\
    \midrule
        $Y$&1\\
        $Q$&1.03\\
        \bottomrule
    \end{tabular}
    \caption{Volatility}
    \label{quantresults2}
\end{minipage}
\end{table}


The model provides 3 main insights: i) the optimal inventories are procyclically adjusted; ii) the assumption that $\alpha$ is a constant is not confirmed by the model with endogenous inventory policy as the observed $\alpha$ is countercyclical, however the optimal $\alpha$ varies in a small range; iii) the model delivers upstream amplification in that the standard deviation of output is larger than the one of sales. 

Note that an extension with more than one firm in a sequential production setting would immediately deliver upstream amplification of demand shocks as an intermediate good firm would face the final good producer output policy as demand process. As the final good firm output policy is more volatile than final demand, additional firms upstream would face ever increasing volatility.

I conclude that, while obviously an approximation, the maintained assumption of exogenous inventory policy can be partially rationalised through a model in which firms face a time to sell constrained and a penalty if they do not meet demand.
